Quantum CPOs

We introduce the monoidal closed category qCPO of quantum cpos, whose objects are "quantized" analogs of omega-complete partial orders (cpos). The category qCPO is enriched over the category CPO of cpos, and contains both CPO, and the opposite of the category FdAlg of finite-dimensional von Neumann algebras as monoidal subcategories. We use qCPO to construct a sound model for the quantum programming language Proto-Quipper-M (PQM) extended with term recursion, as well as a sound and computationally adequate model for the Linear/Non-Linear Fixpoint Calculus (LNL-FPC), which is both an extension of the Fixpoint Calculus (FPC) with linear types, and an extension of a circuit-free fragment of PQM that includes recursive types.

==> eptcsdata.tex <==
\providecommand{\firstpage}{174}
\providecommand{\publicationstatus}{B. Valiron, S. Mansfield, P. Arrighi and P. Panangaden\\ (Eds.): Quantum Physics and Logic 2020 (QPL'20)\\
EPTCS 340, 2021, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.340.9}{10.4204/EPTCS.340.9}}
\pdfoutput=1

